Unrealized Expectations: Comparing AI Methods vs Classical Algorithms for Maximum Independent Set

AI methods, such as generative models and reinforcement learning, have recently been applied to combinatorial optimization (CO) problems, especially NP-hard ones. This paper compares such GPU-based methods with classical CPU-based methods on the Maximum Independent Set (MIS) problem. Strikingly, even on in-distribution random graphs, leading AI-inspired methods are consistently outperformed by the state-of-the-art classical solver KaMIS running on a single CPU, and some AI-inspired methods frequently fail to surpass even the simplest degree-based greedy heuristic. Even with post-processing techniques like local search, AI-inspired methods still perform worse than CPU-based solvers. To better understand the source of these failures, we introduce a novel analysis, serialization, which reveals that non-backtracking AI-inspired methods, e.g. LTFT (which is based on GFlowNets), end up reasoning similarly to the simplest degree-based greedy, and thus worse than KaMIS. More generally, our findings suggest a need for a rethinking of current approaches in AI for CO, advocating for more rigorous benchmarking and the principled integration of classical heuristics. Additionally, we also find that CPU-based algorithm KaMIS have strong performance on sparse random graphs, which appears to show that the shattering threshold conjecture for large independent sets proposed by Coja-Oghlan & Efthymiou (2015) does not apply for real-life sizes (such as 10^6 nodes).

==> conjecture.tex <==
\section{Perspective for theoreticians: Does \kamis refutes famous conjecture?}\label{sec:refute-conjecture_app}
For theoretical analysis for MIS on ER graphs and regular graphs, see~\citet{coja2015independent, wormald1999differential, barbier2013hard, gamarnik2014limits}. In ER graphs with $n$ nodes and average degree $d$, the  MIS has size $\frac{2n\ln d}{d}$ for asymptotically large $n$ and $d$, and simplest random greedy  achieves half-optimal at $\frac{n\ln d}{d}$~\citep{grimmett1975colouring}. Yet, there is no known polynomial-time algorithm which can achieve MIS size $(1+\eps)\frac{n\ln d}{d}$ for any constant $\eps$ and it is conjectured that polynomial-time algorithms cannot do better than  $(1+o(1))\frac{n\ln d}{d}$~\citep{coja2015independent}.  Thus it is natural to measure the goodness of an algorithm by the ratio of the MIS size obtained to $\frac{n\ln d}{d}$. This ratio can faciliate comparison across different $n$ and $d$'s.

\Cref{fig:er_heatmap} shows the ratio of MIS size to $\frac{n\ln d}{d}$ for ER graphs with number of nodes $n$ and average degree $d$ across various algorithms. Surprisingly  for \redumis and \onlinemis this ratio is consistently larger than $1.2$ and often larger than $1.3$ even for fairly large $n, d$.  These results seem to bring the conjecture in doubt, but not disprove per se since the conjecture concerns asymptotically large $n$ and $d$. But  our results could encourage further analysis and potential collaboration between researchers on theoretical and empirical aspects of MIS on random graphs.

\input{figs/fig_gnm_heatmap}

%We can see that \redumis, \onlinemis, and \isco has consitently high ratios more than $1.2$. \rangreedy stays around $1.0$ for all $(n,d)$. Other algorithms, including \deggreedy, all have higher ratios for sparser graphs, but lower ratios (close to $1$) for denser graphs.

